MAFER: a Multi-resolution Approach to Facial Expression Recognition

Emotions play a central role in the social life of every human being, and their study, which represents a multidisciplinary subject, embraces a great variety of research fields. Especially concerning the latter, the analysis of facial expressions represents a very active research area due to its relevance to human-computer interaction applications. In such a context, Facial Expression Recognition (FER) is the task of recognizing expressions on human faces. Typically, face images are acquired by cameras that have, by nature, different characteristics, such as the output resolution. It has been already shown in the literature that Deep Learning models applied to face recognition experience a degradation in their performance when tested against multi-resolution scenarios. Since the FER task involves analyzing face images that can be acquired with heterogeneous sources, thus involving images with different quality, it is plausible to expect that resolution plays an important role in such a case too. Stemming from such a hypothesis, we prove the benefits of multi-resolution training for models tasked with recognizing facial expressions. Hence, we propose a two-step learning procedure, named MAFER, to train DCNNs to empower them to generate robust predictions across a wide range of resolutions. A relevant feature of MAFER is that it is task-agnostic, i.e., it can be used complementarily to other objective-related techniques. To assess the effectiveness of the proposed approach, we performed an extensive experimental campaign on publicly available datasets: \fer{}, \raf{}, and \oulu{}. For a multi-resolution context, we observe that with our approach, learning models improve upon the current SotA while reporting comparable results in fix-resolution contexts. Finally, we analyze the performance of our models and observe the higher discrimination power of deep features generated from them.

==> tables/cbir_oulu_map.tex <==
\begin{table}[!h]
    \centering
    \begin{tabularx}{0.7\linewidth}{l>{\centering\arraybackslash}X}
    \toprule
    \textbf{Model} & \textbf{mAP (\%)} \\
    \cmidrule{1-2} 
    
    base & 35.43 $\pm$ 1.09 \\
    \\
    MAFAR & \\
    \cmidrule{1-1} 
    CR &  70.75 $\pm$ 1.53 \\
    CR-Simiplified  & 78.61 $\pm$ 1.53  \\
    CR+AffWild2  &  79.58 $\pm$ 1.67\\ 
    
    \bottomrule
    \end{tabularx}
  \caption{mAP for the \oulu{} dataset.} 
   \label{tab:cbir_oulu_map}
\end{table}

==> tables/cbir_oulu_rec.tex <==
\begin{table*}
\centering
\begin{tabularx}{\linewidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
\toprule
& & \multicolumn{7}{c}{\textbf{Recall@k (\%)}} \\
\cmidrule{3-9} 
\textbf{Model} & &  1 & 5 & 10 & 50 & 100 & 300 & 500 \\ 
\hline

base          & &  0.42 $\pm$ .02 & 1.70 $\pm$ .07 & 3.06 $\pm$ .13 & 12.43 $\pm$ .46 & 21.52 $\pm$ .74 & 46.79 $\pm$ 1.11 & 65.40 $\pm$ 1.07 \\ 

\\
MAFAR & & & & & & & & \\ \cmidrule{1-1} 

CR            & & 0.48 $\pm$ .01 & 2.33 $\pm$ .05 & 4.54 $\pm$ .11 & 21.36 $\pm$ .64 & 40.70 $\pm$ 1.26 & 74.72 $\pm$ 1.83 & 84.18 $\pm$ 1.39 \\

CR-Simplified &  &  0.51 $\pm$ .00 & 2.49 $\pm$ .02 & 4.90 $\pm$ .05 & 23.16 $\pm$ .46 & 44.55 $\pm$ 1.04 & 81.99 $\pm$ 1.11 & 87.68 $\pm$ .75 \\

CR+AffWild2   & &  0.50 $\pm$ .00 & 2.49 $\pm$ .02 & 4.94 $\pm$ .05 & 23.67 $\pm$ .34 & 45.27 $\pm$ .81 & 82.04 $\pm$ 1.39 & 89.07 $\pm$ 1.01 \\

\bottomrule
\end{tabularx}
\caption{Recall@k for the \oulu{} dataset. Each value is the average among 20 queries.}
\label{tab:cbir_oulu_rec}
\end{table*}


==> tables/expw.tex <==

\begin{table}[]
    \centering
    \begin{tabularx}{\linewidth}{l>{\centering\arraybackslash}X}
    \toprule
    \textbf{Authors} & \textbf{Accuracy (\%)} \\ 
    \cmidrule{1-2}
    Lian et al.~\cite{expwresult} (5-fold avg) & 71.90 \\
    Bishay et al.~\cite{bishay2019expw} & 73.10 \\
    Mahmoudi et al.~\cite{mahmoudiexp2} & 76.81 \\
    base & \\
    \\
    MAFAR & \\
    \cmidrule{1-1} 
    CR &  \\
    CR-Simiplified & \\
    CR+AffWild2  &  \\
    \bottomrule
    \multicolumn{2}{@{}l}{$^\star$10-fold Averaged}\\ 
    \end{tabularx}
    \caption{ExpW~\cite{expw} dataset}
    \label{tab:expw}
\end{table}
